Efficient and Effective Local Search for the Set-Union Knapsack Problem and Budgeted Maximum Coverage Problem

The Set-Union Knapsack Problem (SUKP) and Budgeted Maximum Coverage Problem (BMCP) are two closely related variant problems of the popular knapsack problem. Given a set of weighted elements and a set of items with nonnegative values, where each item covers several distinct elements, these two problems both aim to find a subset of items that maximizes an objective function while satisfying a knapsack capacity (budget) constraint. We propose an efficient and effective local search algorithm called E2LS for these two problems. To our knowledge, this is the first time that an algorithm has been proposed for both of them. E2LS trade-offs the search region and search efficiency by applying a proposed novel operator ADD$^*$ to traverse the refined search region. Such a trade-off mechanism allows E2LS to explore the solution space widely and quickly. The tabu search method is also applied in E2LS to help the algorithm escape from local optima. Extensive experiments on a total of 168 public instances with various scales demonstrate the excellent performance of the proposed algorithm for both the SUKP and BMCP.

==> table-BMCP-new.tex <==
\begin{table*}[t]
\caption{Comparison of E2LS with the baseline algorithms on all the three sets of BMCP instances. Unique/Equal best results appear in bold/italic.}
\label{table-BMCP}
\centering
\scalebox{0.59}{\begin{tabular}{lrrrrrrrrrrr} \toprule
Instance\textbackslash{}Algorithm &  & \multicolumn{2}{r}{PLTS}     &  & \multicolumn{2}{r}{VDLS}               &           & \multicolumn{4}{r}{E2LS}                                    \\ \cline{3-4} \cline{6-7} \cline{9-12} 
                                  &  & Best            & Average    &  & Best              & Average            &           & Best                & Average             & S.D.  & Time    \\ \hline
\textit{\textit{Set A}}                    &  &                 &            &  &                   &                    &           &                     &                     &       &         \\ \hline
bmcp\_585\_600\_0.05\_2000        &  & 70997           & 70892.60   &  & \textit{71102}    & 71034.37           &           & \textit{71102}      & \textbf{71102.00}   & 0.00  & 0.525   \\
bmcp\_585\_600\_0.075\_1500       &  & 70677           & 70535.90   &  & \textit{71025}    & 70492.53           &           & \textit{71025}      & \textbf{71025.00}   & 0.00  & 0.729   \\
bmcp\_600\_585\_0.05\_2000        &  & 67187           & 66807.10   &  & \textit{67636}    & 67621.60           &           & \textit{67636}      & \textbf{67636.00}   & 0.00  & 0.317   \\
bmcp\_600\_585\_0.075\_1500       &  & 70318           & 70318.00   &  & \textit{70588}    & 70277.00           &           & \textit{70588}      & \textbf{70588.00}   & 0.00  & 2.357   \\
bmcp\_600\_600\_0.05\_2000        &  & 68453           & 68346.60   &  & \textit{68738}    & 68580.70           &           & \textit{68738}      & \textbf{68738.00}   & 0.00  & 0.419   \\
bmcp\_600\_600\_0.075\_1500       &  & 71746           & 71746.00   &  & \textit{71904}    & 71780.73           &           & \textit{71904}      & \textbf{71904.00}   & 0.00  & 0.476   \\
bmcp\_685\_700\_0.05\_2000        &  & 80111           & 79979.90   &  & \textit{81227}    & 80482.47           &           & \textit{81227}      & \textbf{81227.00}   & 0.00  & 0.593   \\
bmcp\_685\_700\_0.075\_1500       &  & 82955           & 82933.40   &  & \textit{83286}    & 82886.63           &           & \textit{83286}      & \textbf{83286.00}   & 0.00  & 2.024   \\
bmcp\_700\_685\_0.05\_2000        &  & \textit{78054}  & 77460.80   &  & \textit{78054}    & 77742.87           &           & \textit{78054}      & \textbf{78054.00}   & 0.00  & 0.365   \\
bmcp\_700\_685\_0.075\_1500       &  & \textit{78869}  & 78580.10   &  & \textit{78869}    & 78642.90           &           & \textit{78869}      & \textbf{78869.00}   & 0.00  & 0.487   \\
bmcp\_700\_700\_0.05\_2000        &  & 77424           & 77225.80   &  & \textit{78458}    & 78180.40           &           & \textit{78458}      & \textbf{78458.00}   & 0.00  & 0.335   \\
bmcp\_700\_700\_0.075\_1500       &  & 84570           & 83406.50   &  & \textit{84576}    & \textit{84576.00}  &           & \textit{84576}      & \textit{84576.00}   & 0.00  & 0.313   \\
bmcp\_785\_800\_0.05\_2000        &  & 92505           & 92080.70   &  & \textit{92740}    & 92414.17           &           & \textit{92740}      & \textbf{92740.00}   & 0.00  & 20.643  \\
bmcp\_785\_800\_0.075\_1500       &  & 94245           & 94243.80   &  & \textit{95221}    & \textit{95221.00}  & \textit{} & \textit{95221}      & \textit{95221.00}   & 0.00  & 0.692   \\
bmcp\_800\_785\_0.05\_2000        &  & 88562           & 88424.30   &  & \textit{89138}    & 89054.73           &           & \textit{89138}      & \textbf{89138.00}   & 0.00  & 0.401   \\
bmcp\_800\_785\_0.075\_1500       &  & 91021           & 90888.90   &  & \textit{91856}    & 91722.93           &           & \textit{91856}      & \textbf{91856.00}   & 0.00  & 0.612   \\
bmcp\_800\_800\_0.05\_2000        &  & 90951           & 90697.40   &  & \textit{91795}    & 91572.83           &           & \textit{91795}      & \textbf{91795.00}   & 0.00  & 2.210   \\
bmcp\_800\_800\_0.075\_1500       &  & 95533           & 95508.80   &  & \textit{95995}    & 95568.47           &           & \textit{95995}      & \textbf{95995.00}   & 0.00  & 6.586   \\
bmcp\_885\_900\_0.05\_2000        &  & 101293          & 100857.00  &  & \textit{102277}   & 102059.17          &           & \textit{102277}     & \textbf{102277.00}  & 0.00  & 0.392   \\
bmcp\_885\_900\_0.075\_1500       &  & 105718          & 105707.70  &  & \textit{106940}   & 106446.90          &           & \textit{106940}     & \textbf{106940.00}  & 0.00  & 1.264   \\
bmcp\_900\_885\_0.05\_2000        &  & 98840           & 98485.50   &  & \textit{99590}    & 99365.10           &           & \textit{99590}      & \textbf{99590.00}   & 0.00  & 0.455   \\
bmcp\_900\_885\_0.075\_1500       &  & 103596          & 103223.10  &  & \textit{105141}   & 105024.80          &           & \textit{105141}     & \textbf{105141.00}  & 0.00  & 0.420   \\
bmcp\_900\_900\_0.05\_2000        &  & 101265          & 101210.70  &  & \textit{102055}   & 101402.60          &           & \textit{102055}     & \textbf{102055.00}  & 0.00  & 0.610   \\
bmcp\_900\_900\_0.075\_1500       &  & 104521          & 104521.00  &  & \textit{105081}   & 104919.10          &           & \textit{105081}     & \textbf{105081.00}  & 0.00  & 0.553   \\
bmcp\_985\_1000\_0.05\_2000       &  & 109523          & 108681.80  &  & \textit{110669}   & 109792.57          &           & \textit{110669}     & \textbf{110669.00}  & 0.00  & 0.782   \\
bmcp\_985\_1000\_0.075\_1500      &  & 113541          & 113439.40  &  & \textit{115505}   & 114765.27          &           & \textit{115505}     & \textbf{115505.00}  & 0.00  & 0.519   \\
bmcp\_1000\_985\_0.05\_2000       &  & 111212          & 110379.10  &  & \textit{112057}   & 111583.10          &           & \textit{112057}     & \textbf{112057.00}  & 0.00  & 33.772  \\
bmcp\_1000\_985\_0.075\_1500      &  & 112250          & 112160.20  &  & \textit{113615}   & 113096.13          &           & \textit{113615}     & \textbf{113615.00}  & 0.00  & 0.535   \\
bmcp\_1000\_1000\_0.05\_2000      &  & 111829          & 111318.60  &  & \textit{113331}   & 113124.77          &           & \textit{113331}     & \textbf{113331.00}  & 0.00  & 0.446   \\
bmcp\_1000\_1000\_0.075\_1500     &  & 118244          & 118243.10  &  & \textit{120246}   & 119994.53          &           & \textit{120246}     & \textbf{120246.00}  & 0.00  & 0.449   \\
Average                           &  & 91533.67        & 91276.79   &  & \textit{92290.50} & 91980.88           &           & \textit{92290.50}   & \textbf{92290.50}   & 0.00  & 2.676   \\ \hline
\textit{\textit{Set B}}                    &  &                 &            &  &                   &                    &           &                     &                     &       &         \\ \hline
bmcp\_1100\_1000\_0.3\_3000       &  & 142835          & 142428.70  &  & \textit{143475}   & 143224.60          &           & \textit{143475}     & \textbf{143475.00}  & 0.00  & 1.111   \\
bmcp\_1100\_1000\_0.5\_2000       &  & 125974          & 125790.00  &  & 126917            & 126021.57          &           & \textbf{127157}     & \textbf{127157.00}  & 0.00  & 0.839   \\
bmcp\_1100\_1100\_0.3\_3000       &  & 154936          & 154661.70  &  & \textit{157530}   & 156462.53          &           & \textit{157530}     & \textbf{157530.00}  & 0.00  & 1.006   \\
bmcp\_1100\_1100\_0.5\_2000       &  & 139196          & 138169.00  &  & 139141            & 138719.40          &           & \textbf{139235}     & \textbf{139235.00}  & 0.00  & 1.813   \\
bmcp\_1100\_1200\_0.3\_3000       &  & 169113          & 168763.60  &  & \textit{172660}   & 172075.30          &           & \textit{172660}     & \textbf{172660.00}  & 0.00  & 0.442   \\
bmcp\_1100\_1200\_0.5\_2000       &  & 150301          & 149366.40  &  & \textit{150493}   & 149944.03          &           & \textit{150493}     & \textbf{150493.00}  & 0.00  & 0.636   \\
bmcp\_1200\_1100\_0.3\_3000       &  & \textit{161848} & 159620.30  &  & \textit{161848}   & \textit{161848.00} & \textit{} & \textit{161848}     & \textit{161848.00}  & 0.00  & 0.317   \\
bmcp\_1200\_1100\_0.5\_2000       &  & 135858          & 135509.20  &  & \textit{137700}   & 136831.20          &           & \textit{137700}     & \textbf{137700.00}  & 0.00  & 5.991   \\
bmcp\_1200\_1200\_0.3\_3000       &  & 169219          & 168821.70  &  & \textit{172595}   & 172151.83          &           & \textit{172595}     & \textbf{172595.00}  & 0.00  & 0.847   \\
bmcp\_1200\_1200\_0.5\_2000       &  & 149654          & 148679.10  &  & \textit{151440}   & 149609.97          &           & \textit{151440}     & \textbf{151440.00}  & 0.00  & 2.472   \\
bmcp\_1200\_1300\_0.3\_3000       &  & 183004          & 182220.40  &  & \textit{186083}   & 183599.00          &           & \textit{186083}     & \textbf{186083.00}  & 0.00  & 7.467   \\
bmcp\_1200\_1300\_0.5\_2000       &  & 160369          & 159735.40  &  & \textit{162154}   & 161146.93          &           & \textit{162154}     & \textbf{162154.00}  & 0.00  & 5.028   \\
bmcp\_1300\_1200\_0.3\_3000       &  & 168586          & 168473.80  &  & \textit{170786}   & 169724.67          &           & \textit{170786}     & \textbf{170786.00}  & 0.00  & 22.551  \\
bmcp\_1300\_1200\_0.5\_2000       &  & 151067          & 150034.70  &  & 151402            & 151049.43          &           & \textbf{151512}     & \textbf{151512.00}  & 0.00  & 10.943  \\
bmcp\_1300\_1300\_0.3\_3000       &  & 180608          & 179978.40  &  & \textit{184699}   & 183239.03          &           & \textit{184699}     & \textbf{184699.00}  & 0.00  & 7.728   \\
bmcp\_1300\_1300\_0.5\_2000       &  & 160485          & 159511.30  &  & 162146            & 161536.70          &           & \textbf{162514}     & \textbf{162514.00}  & 0.00  & 43.851  \\
bmcp\_1300\_1400\_0.3\_3000       &  & 197709          & 195681.90  &  & \textit{199134}   & 198889.43          &           & \textit{199134}     & \textbf{199134.00}  & 0.00  & 0.412   \\
bmcp\_1300\_1400\_0.5\_2000       &  & 173349          & 171665.00  &  & \textit{173954}   & 173799.23          &           & \textit{173954}     & \textbf{173954.00}  & 0.00  & 4.857   \\
bmcp\_1400\_1300\_0.3\_3000       &  & 182881          & 180143.50  &  & 183987            & 183796.30          &           & \textbf{184691}     & \textbf{184691.00}  & 0.00  & 238.817 \\
bmcp\_1400\_1300\_0.5\_2000       &  & 161995          & 160647.00  &  & \textit{162544}   & 162312.87          &           & \textit{162544}     & \textbf{162544.00}  & 0.00  & 35.752  \\
bmcp\_1400\_1400\_0.3\_3000       &  & 199879          & 197229.00  &  & \textit{200136}   & 199616.67          &           & \textit{200136}     & \textbf{200136.00}  & 0.00  & 1.883   \\
bmcp\_1400\_1400\_0.5\_2000       &  & 174683          & 173393.10  &  & \textit{175583}   & 173984.93          &           & \textit{175583}     & \textbf{175583.00}  & 0.00  & 83.975  \\
bmcp\_1400\_1500\_0.3\_3000       &  & 210077          & 208315.60  &  & \textit{212492}   & 211264.37          &           & \textit{212492}     & \textbf{212492.00}  & 0.00  & 59.715  \\
bmcp\_1400\_1500\_0.5\_2000       &  & 184259          & 183289.90  &  & \textit{186818}   & 186250.33          &           & \textit{186818}     & \textbf{186818.00}  & 0.00  & 9.601   \\
bmcp\_1500\_1400\_0.3\_3000       &  & 194156          & 193554.80  &  & 197219            & 196703.40          &           & \textbf{197899}     & \textbf{197899.00}  & 0.00  & 210.823 \\
bmcp\_1500\_1400\_0.5\_2000       &  & 173475          & 171426.90  &  & 174284            & 173576.40          &           & \textbf{174522}     & \textbf{174522.00}  & 0.00  & 67.331  \\
bmcp\_1500\_1500\_0.3\_3000       &  & 209929          & 207795.30  &  & \textit{211108}   & 210393.73          &           & \textit{211108}     & \textbf{211108.00}  & 0.00  & 1.910   \\
bmcp\_1500\_1500\_0.5\_2000       &  & 184082          & 182676.20  &  & \textit{187052}   & 185221.60          &           & \textit{187052}     & \textbf{187052.00}  & 0.00  & 2.435   \\
bmcp\_1500\_1600\_0.3\_3000       &  & \textit{226408} & 221641.30  &  & \textit{226408}   & 224926.60          &           & \textit{226408}     & \textbf{226408.00}  & 0.00  & 2.314   \\
bmcp\_1500\_1600\_0.5\_2000       &  & 198214          & 196659.00  &  & \textit{199678}   & 198462.63          &           & \textit{199678}     & \textbf{199678.00}  & 0.00  & 87.173  \\
Average                           &  & 172471.63       & 171196.07  &  & 174048.87         & 173212.76          &           & \textbf{174130.00}  & \textbf{174130.00}  & 0.00  & 30.668  \\ \hline
\textit{\textit{Set C}}                    &  &                 &            &  &                   &                    &           &                     &                     &       &         \\ \hline
bmcp\_4200\_4000\_0.3\_10000      &  & 1778013         & 1747411.90 &  & \textit{1835947}  & 1833108.20         &           & \textit{1835947}    & \textbf{1835947.00} & 0.00  & 5.636   \\
bmcp\_4200\_4000\_0.5\_7000       &  & 1685141         & 1666673.30 &  & \textit{1738553}  & 1729188.00         &           & \textit{1738553}    & \textbf{1738553.00} & 0.00  & 17.241  \\
bmcp\_4200\_4200\_0.3\_10000      &  & 1874190         & 1839780.10 &  & 1925706           & 1918624.23         &           & \textbf{1925859}    & \textbf{1925859.00} & 0.00  & 3.422   \\
bmcp\_4200\_4200\_0.5\_7000       &  & 1764277         & 1742121.70 &  & 1811649           & 1801880.20         &           & \textbf{1816714}    & \textbf{1816714.00} & 0.00  & 23.069  \\
bmcp\_4200\_4400\_0.3\_10000      &  & 1954069         & 1932251.00 &  & \textit{2023093}  & 2020209.80         &           & \textit{2023093}    & \textbf{2023093.00} & 0.00  & 21.845  \\
bmcp\_4200\_4400\_0.5\_7000       &  & 1853677         & 1820444.40 &  & \textit{1903515}  & 1889809.53         &           & \textit{1903515}    & \textbf{1903515.00} & 0.00  & 17.612  \\
bmcp\_4400\_4200\_0.3\_10000      &  & 1833465         & 1816879.10 &  & \textit{1920418}  & 1911396.17         &           & \textit{1920418}    & \textbf{1920418.00} & 0.00  & 25.126  \\
bmcp\_4400\_4200\_0.5\_7000       &  & 1746064         & 1730783.90 &  & 1810031           & 1805200.73         &           & \textbf{1811179}    & \textbf{1811179.00} & 0.00  & 44.223  \\
bmcp\_4400\_4400\_0.3\_10000      &  & 1945218         & 1922134.20 &  & 2027801           & 2024036.13         &           & \textbf{2028288}    & \textbf{2028288.00} & 0.00  & 4.064   \\
bmcp\_4400\_4400\_0.5\_7000       &  & 1844031         & 1821467.80 &  & 1901941           & 1888300.50         &           & \textbf{1905810}    & \textbf{1905810.00} & 0.00  & 68.641  \\
bmcp\_4400\_4600\_0.3\_10000      &  & 2003959         & 1993946.20 &  & \textit{2100925}  & 2093610.13         &           & \textit{2100925}    & \textbf{2100925.00} & 0.00  & 6.291   \\
bmcp\_4400\_4600\_0.5\_7000       &  & 1937066         & 1906956.10 &  & 1989582           & 1979416.63         &           & \textbf{1991870}    & \textbf{1991870.00} & 0.00  & 8.372   \\
bmcp\_4600\_4400\_0.3\_10000      &  & 1930498         & 1913501.00 &  & 2008258           & 2001368.77         &           & \textbf{2011730}    & \textbf{2011730.00} & 0.00  & 11.351  \\
bmcp\_4600\_4400\_0.5\_7000       &  & 1845046         & 1817697.20 &  & 1898602           & 1889658.47         &           & \textbf{1901868}    & \textbf{1901868.00} & 0.00  & 97.821  \\
bmcp\_4600\_4600\_0.3\_10000      &  & 2027132         & 2005096.70 &  & 2106938           & 2100124.47         &           & \textbf{2106970}    & \textbf{2106970.00} & 0.00  & 7.914   \\
bmcp\_4600\_4600\_0.5\_7000       &  & 1921261         & 1900376.30 &  & 1980462           & 1973677.23         &           & \textbf{1984295}    & \textbf{1984295.00} & 0.00  & 41.538  \\
bmcp\_4600\_4800\_0.3\_10000      &  & 2120120         & 2091722.50 &  & 2201977           & 2197572.40         &           & \textbf{2203833}    & \textbf{2203833.00} & 0.00  & 18.406  \\
bmcp\_4600\_4800\_0.5\_7000       &  & 1989454         & 1967943.30 &  & 2070913           & 2057914.30         &           & \textbf{2074036}    & \textbf{2074036.00} & 0.00  & 22.452  \\
bmcp\_4800\_4600\_0.3\_10000      &  & 2019033         & 1991673.50 &  & 2096747           & 2087481.97         &           & \textbf{2101148}    & \textbf{2101148.00} & 0.00  & 10.699  \\
bmcp\_4800\_4600\_0.5\_7000       &  & 1922466         & 1901157.60 &  & 1991409           & 1973721.93         &           & \textbf{1992370}    & \textbf{1992370.00} & 0.00  & 109.582 \\
bmcp\_4800\_4800\_0.3\_10000      &  & 2100773         & 2058921.60 &  & 2183525           & 2175464.77         &           & \textbf{2185367}    & \textbf{2185367.00} & 0.00  & 7.115   \\
bmcp\_4800\_4800\_0.5\_7000       &  & 2009129         & 1973993.60 &  & 2066487           & 2059458.67         &           & \textbf{2075133}    & \textbf{2075133.00} & 0.00  & 346.026 \\
bmcp\_4800\_5000\_0.3\_10000      &  & 2184445         & 2157793.00 &  & \textit{2280317}  & 2273869.03         &           & \textit{2280317}    & \textbf{2280317.00} & 0.00  & 3.414   \\
bmcp\_4800\_5000\_0.5\_7000       &  & 2087596         & 2050741.00 &  & 2146413           & 2136313.23         &           & \textbf{2151715}    & \textbf{2151715.00} & 0.00  & 203.314 \\
bmcp\_5000\_4800\_0.3\_10000      &  & 2069979         & 2051607.20 &  & 2183483           & 2175171.23         &           & \textbf{2184508}    & \textbf{2184508.00} & 0.00  & 11.619  \\
bmcp\_5000\_4800\_0.5\_7000       &  & 2013921         & 1977310.70 &  & 2066000           & 2053359.87         &           & \textbf{2070324}    & \textbf{2070305.90} & 54.30 & 468.996 \\
bmcp\_5000\_5000\_0.3\_10000      &  & 2144223         & 2126462.90 &  & \textit{2261620}  & 2251526.97         &           & \textit{2261620}    & \textbf{2261620.00} & 0.00  & 107.113 \\
bmcp\_5000\_5000\_0.5\_7000       &  & 2067188         & 2046886.50 &  & \textit{2151921}  & 2141828.57         &           & \textit{2151921}    & \textbf{2151921.00} & 0.00  & 32.261  \\
bmcp\_5000\_5200\_0.3\_10000      &  & 2231359         & 2220887.20 &  & \textit{2354408}  & 2345758.73         &           & \textit{2354408}    & \textbf{2354408.00} & 0.00  & 14.278  \\
bmcp\_5000\_5200\_0.5\_7000       &  & 2129556         & 2115338.30 &  & 2222169           & 2211650.90         &           & \textbf{2227362}    & \textbf{2227362.00} & 0.00  & 341.662 \\ \hline
Average                           &  & 1967744.97      & 1943665.33 &  & 2042027.00        & 2033356.73         &           & \textbf{2044036.53} & \textbf{2044035.93} & 1.81  & 70.037 
 \\ \bottomrule
\end{tabular}}
\end{table*}

==> table-BMCP.tex <==
\begin{table*}[t]
\caption{Comparison of E2LS with the baseline algorithms on all the three sets of BMCP instances. Unique/Equal best results appear in bold/italic.}
\label{table-BMCP}
\centering
\scalebox{0.59}{\begin{tabular}{lrrrrrrrrrrr} \toprule
Instance\textbackslash{}Algorithm                                  &  & \multicolumn{2}{r}{PLTS}     &  & \multicolumn{2}{r}{VDLS}              &           & \multicolumn{4}{r}{E2LS}                                    \\ \cline{3-4} \cline{6-7} \cline{9-12} 
                                                                   &  & Best            & Average    &  & Best             & Average            &           & Best                & Average             & S.D.  & Time    \\ \hline
\multicolumn{12}{l}{\textit{Set A}}                                                                                                                                                                                       \\ \hline
bmcp\_585\_600\_0.05\_2000                  &  & 70997           & 70892.60   &  & 71091            & 71006.50           &           & \textbf{71102}      & \textbf{71102.00}   & 0.00  & 0.525   \\
bmcp\_585\_600\_0.075\_1500                 &  & 70677           & 70535.90   &  & \textit{71025}   & 70554.20           &           & \textit{71025}      & \textbf{71025.00}   & 0.00  & 0.729   \\
bmcp\_600\_585\_0.05\_2000                  &  & 67187           & 66807.10   &  & \textit{67636}   & 67621.60           &           & \textit{67636}      & \textbf{67636.00}   & 0.00  & 0.317   \\
bmcp\_600\_585\_0.075\_1500                 &  & 70318           & 70318.00   &  & \textit{70588}   & 70367.10           &           & \textit{70588}      & \textbf{70588.00}   & 0.00  & 2.357   \\
bmcp\_600\_600\_0.05\_2000                  &  & 68453           & 68346.60   &  & \textit{68738}   & 68559.90           &           & \textit{68738}      & \textbf{68738.00}   & 0.00  & 0.419   \\
bmcp\_600\_600\_0.075\_1500                 &  & 71746           & 71746.00   &  & \textit{71904}   & 71833.20           &           & \textit{71904}      & \textbf{71904.00}   & 0.00  & 0.476   \\
bmcp\_685\_700\_0.05\_2000                  &  & 80111           & 79979.90   &  & 80751            & 80388.70           &           & \textbf{81227}      & \textbf{81227.00}   & 0.00  & 0.593   \\
bmcp\_685\_700\_0.075\_1500                 &  & 82955           & 82933.40   &  & \textit{83286}   & 82870.30           &           & \textit{83286}      & \textbf{83286.00}   & 0.00  & 2.024   \\
bmcp\_700\_685\_0.05\_2000                  &  & \textit{78054}  & 77460.80   &  & \textit{78054}   & 77674.40           &           & \textit{78054}      & \textbf{78054.00}   & 0.00  & 0.365   \\
bmcp\_700\_685\_0.075\_1500                 &  & \textit{78869}  & 78580.10   &  & \textit{78869}   & 78649.10           &           & \textit{78869}      & \textbf{78869.00}   & 0.00  & 0.487   \\
bmcp\_700\_700\_0.05\_2000                  &  & 77424           & 77225.80   &  & \textit{78458}   & 78252.70           &           & \textit{78458}      & \textbf{78458.00}   & 0.00  & 0.335   \\
bmcp\_700\_700\_0.075\_1500                 &  & 84570           & 83406.50   &  & \textit{84576}   & 84576.00           &           & \textit{84576}      & \textbf{84576.00}   & 0.00  & 0.313   \\
bmcp\_785\_800\_0.05\_2000                  &  & 92505           & 92080.70   &  & 92630            & 92400.10           &           & \textbf{92740}      & \textbf{92740.00}   & 0.00  & 20.643  \\
bmcp\_785\_800\_0.075\_1500                 &  & 94245           & 94243.80   &  & \textit{95221}   & \textit{95221.00}  & \textit{} & \textit{95221}      & \textit{95221.00}   & 0.00  & 0.692   \\
bmcp\_800\_785\_0.05\_2000                  &  & 88562           & 88424.30   &  & \textit{89138}   & 89024.70           &           & \textit{89138}      & \textbf{89138.00}   & 0.00  & 0.401   \\
bmcp\_800\_785\_0.075\_1500                 &  & 91021           & 90888.90   &  & \textit{91856}   & 91644.60           &           & \textit{91856}      & \textbf{91856.00}   & 0.00  & 0.612   \\
bmcp\_800\_800\_0.05\_2000                  &  & 90951           & 90697.40   &  & \textit{91795}   & 91541.80           &           & \textit{91795}      & \textbf{91795.00}   & 0.00  & 2.210   \\
bmcp\_800\_800\_0.075\_1500                 &  & 95533           & 95508.80   &  & \textit{95995}   & 95652.60           &           & \textit{95995}      & \textbf{95995.00}   & 0.00  & 6.586   \\
bmcp\_885\_900\_0.05\_2000                  &  & 101293          & 100857.00  &  & \textit{102277}  & 101853.20          &           & \textit{102277}     & \textbf{102277.00}  & 0.00  & 0.392   \\
bmcp\_885\_900\_0.075\_1500                 &  & 105718          & 105707.70  &  & \textit{106940}  & 106477.20          &           & \textit{106940}     & \textbf{106940.00}  & 0.00  & 1.264   \\
bmcp\_900\_885\_0.05\_2000                  &  & 98840           & 98485.50   &  & \textit{99590}   & 99289.10           &           & \textit{99590}      & \textbf{99590.00}   & 0.00  & 0.455   \\
bmcp\_900\_885\_0.075\_1500                 &  & 103596          & 103223.10  &  & \textit{105141}  & 104991.60          &           & \textit{105141}     & \textbf{105141.00}  & 0.00  & 0.420   \\
bmcp\_900\_900\_0.05\_2000                  &  & 101265          & 101210.70  &  & 101857           & 101089.20          &           & \textbf{102055}     & \textbf{102055.00}  & 0.00  & 0.610   \\
bmcp\_900\_900\_0.075\_1500                 &  & 104521          & 104521.00  &  & \textit{105081}  & 104955.70          &           & \textit{105081}     & \textbf{105081.00}  & 0.00  & 0.553   \\
bmcp\_985\_1000\_0.05\_2000                 &  & 109523          & 108681.80  &  & 110319           & 109673.10          &           & \textbf{110669}     & \textbf{110669.00}  & 0.00  & 0.782   \\
bmcp\_985\_1000\_0.075\_1500                &  & 113541          & 113439.40  &  & \textit{115505}  & 115075.40          &           & \textit{115505}     & \textbf{115505.00}  & 0.00  & 0.519   \\
bmcp\_1000\_985\_0.05\_2000                 &  & 111212          & 110379.10  &  & \textit{112057}  & 111552.30          &           & \textit{112057}     & \textbf{112057.00}  & 0.00  & 33.772  \\
bmcp\_1000\_985\_0.075\_1500                &  & 112250          & 112160.20  &  & \textit{113615}  & 112984.40          &           & \textit{113615}     & \textbf{113615.00}  & 0.00  & 0.535   \\
bmcp\_1000\_1000\_0.05\_2000                &  & 111829          & 111318.60  &  & \textit{113331}  & 113096.60          &           & \textit{113331}     & \textbf{113331.00}  & 0.00  & 0.446   \\
bmcp\_1000\_1000\_0.075\_1500               &  & 118244          & 118243.10  &  & \textit{120246}  & 119939.30          &           & \textit{120246}     & \textbf{120246.00}  & 0.00  & 0.449   \\ \hline
Average                                                            &  & 91533.67        & 91276.79   &  & 92252.33         & 91960.52           &           & \textbf{92290.50}   & \textbf{92290.50}   & 0.00  & 2.676   \\ \hline
\multicolumn{12}{l}{\textit{Set B}}                                                                                                                                                                                       \\ \hline
bmcp\_1100\_1000\_0.3\_3000  &  & 142835          & 142428.70  &  & 143402           & 143160.20          &           & \textbf{143475}     & \textbf{143475.00}  & 0.00  & 1.111   \\
bmcp\_1100\_1000\_0.5\_2000  &  & 125974          & 125790.00  &  & \textit{127157}  & 126253.10          &           & \textit{127157}     & \textbf{127157.00}  & 0.00  & 0.839   \\
bmcp\_1100\_1100\_0.3\_3000  &  & 154936          & 154661.70  &  & \textit{157530}  & 156962.40          &           & \textit{157530}     & \textbf{157530.00}  & 0.00  & 1.006   \\
bmcp\_1100\_1100\_0.5\_2000  &  & 139196          & 138169.00  &  & 139196           & 138716.50          &           & \textbf{139235}     & \textbf{139235.00}  & 0.00  & 1.813   \\
bmcp\_1100\_1200\_0.3\_3000  &  & 169113          & 168763.60  &  & \textit{172660}  & 172114.00          &           & \textit{172660}     & \textbf{172660.00}  & 0.00  & 0.442   \\
bmcp\_1100\_1200\_0.5\_2000  &  & 150301          & 149366.40  &  & \textit{150493}  & 150043.90          &           & \textit{150493}     & \textbf{150493.00}  & 0.00  & 0.636   \\
bmcp\_1200\_1100\_0.3\_3000  &  & \textit{161848} & 159620.30  &  & \textit{161848}  & \textit{161848.00} & \textit{} & \textit{161848}     & \textit{161848.00}  & 0.00  & 0.317   \\
bmcp\_1200\_1100\_0.5\_2000  &  & 135858          & 135509.20  &  & \textit{137700}  & 136765.60          &           & \textit{137700}     & \textbf{137700.00}  & 0.00  & 5.991   \\
bmcp\_1200\_1200\_0.3\_3000  &  & 169219          & 168821.70  &  & \textit{172595}  & 172081.10          &           & \textit{172595}     & \textbf{172595.00}  & 0.00  & 0.847   \\
bmcp\_1200\_1200\_0.5\_2000  &  & 149654          & 148679.10  &  & 149902           & 149334.40          &           & \textbf{151440}     & \textbf{151440.00}  & 0.00  & 2.472   \\
bmcp\_1200\_1300\_0.3\_3000  &  & 183004          & 182220.40  &  & 184431           & 183686.80          &           & \textbf{186083}     & \textbf{186083.00}  & 0.00  & 7.467   \\
bmcp\_1200\_1300\_0.5\_2000  &  & 160369          & 159735.40  &  & 161662           & 161074.50          &           & \textbf{162154}     & \textbf{162154.00}  & 0.00  & 5.028   \\
bmcp\_1300\_1200\_0.3\_3000  &  & 168586          & 168473.80  &  & 170283           & 169800.50          &           & \textbf{170786}     & \textbf{170786.00}  & 0.00  & 22.551  \\
bmcp\_1300\_1200\_0.5\_2000  &  & 151067          & 150034.70  &  & \textit{151512}  & 151053.20          &           & \textit{151512}     & \textbf{151512.00}  & 0.00  & 10.943  \\
bmcp\_1300\_1300\_0.3\_3000  &  & 180608          & 179978.40  &  & \textit{184699}  & 183427.80          &           & \textit{184699}     & \textbf{184699.00}  & 0.00  & 7.728   \\
bmcp\_1300\_1300\_0.5\_2000  &  & 160485          & 159511.30  &  & 162146           & 161523.80          &           & \textbf{162514}     & \textbf{162514.00}  & 0.00  & 43.851  \\
bmcp\_1300\_1400\_0.3\_3000  &  & 197709          & 195681.90  &  & \textit{199134}  & 198913.40          &           & \textit{199134}     & \textbf{199134.00}  & 0.00  & 0.412   \\
bmcp\_1300\_1400\_0.5\_2000  &  & 173349          & 171665.00  &  & \textit{173954}  & 173773.50          &           & \textit{173954}     & \textbf{173954.00}  & 0.00  & 4.857   \\
bmcp\_1400\_1300\_0.3\_3000  &  & 182881          & 180143.50  &  & 184148           & 183536.20          &           & \textbf{184691}     & \textbf{184691.00}  & 0.00  & 238.817 \\
bmcp\_1400\_1300\_0.5\_2000  &  & 161995          & 160647.00  &  & \textit{162544}  & 162324.70          &           & \textit{162544}     & \textbf{162544.00}  & 0.00  & 35.752  \\
bmcp\_1400\_1400\_0.3\_3000  &  & 199879          & 197229.00  &  & \textit{200136}  & 199714.50          &           & \textit{200136}     & \textbf{200136.00}  & 0.00  & 1.883   \\
bmcp\_1400\_1400\_0.5\_2000  &  & 174683          & 173393.10  &  & \textit{175583}  & 174370.20          &           & \textit{175583}     & \textbf{175583.00}  & 0.00  & 83.975  \\
bmcp\_1400\_1500\_0.3\_3000  &  & 210077          & 208315.60  &  & \textit{212492}  & 211356.60          &           & \textit{212492}     & \textbf{212492.00}  & 0.00  & 59.715  \\
bmcp\_1400\_1500\_0.5\_2000  &  & 184259          & 183289.90  &  & \textit{186818}  & 185991.70          &           & \textit{186818}     & \textbf{186818.00}  & 0.00  & 9.601   \\
bmcp\_1500\_1400\_0.3\_3000  &  & 194156          & 193554.80  &  & \textit{197899}  & 196753.80          &           & \textit{197899}     & \textbf{197899.00}  & 0.00  & 210.823 \\
bmcp\_1500\_1400\_0.5\_2000  &  & 173475          & 171426.90  &  & \textit{174522}  & 173745.10          &           & \textit{174522}     & \textbf{174522.00}  & 0.00  & 67.331  \\
bmcp\_1500\_1500\_0.3\_3000  &  & 209929          & 207795.30  &  & \textit{211108}  & 210451.10          &           & \textit{211108}     & \textbf{211108.00}  & 0.00  & 1.910   \\
bmcp\_1500\_1500\_0.5\_2000  &  & 184082          & 182676.20  &  & \textit{187052}  & 185464.70          &           & \textit{187052}     & \textbf{187052.00}  & 0.00  & 2.435   \\
bmcp\_1500\_1600\_0.3\_3000  &  & \textit{226408} & 221641.30  &  & \textit{226408}  & 225031.90          &           & \textit{226408}     & \textbf{226408.00}  & 0.00  & 2.314   \\
bmcp\_1500\_1600\_0.5\_2000  &  & 198214          & 196659.00  &  & 198579           & 198258.00          &           & \textbf{199678}     & \textbf{199678.00}  & 0.00  & 87.173  \\ \hline
Average                                                            &  & 172471.63       & 171196.07  &  & 173919.77        & 173251.04          &           & \textbf{174130.00}  & \textbf{174130.00}  & 0.00  & 30.668  \\ \hline
\multicolumn{12}{l}{\textit{Set C}}                                                                                                                                                                                       \\ \hline
bmcp\_4200\_4000\_0.3\_10000 &  & 1778013         & 1747411.90 &  & \textit{1835947} & 1828442.40         &           & \textit{1835947}    & \textbf{1835947.00} & 0.00  & 5.636   \\
bmcp\_4200\_4000\_0.5\_7000  &  & 1685141         & 1666673.30 &  & 1733033          & 1724198.80         &           & \textbf{1738553}    & \textbf{1738553.00} & 0.00  & 17.241  \\
bmcp\_4200\_4200\_0.3\_10000 &  & 1874190         & 1839780.10 &  & 1922985          & 1915332.40         &           & \textbf{1925859}    & \textbf{1925859.00} & 0.00  & 3.422   \\
bmcp\_4200\_4200\_0.5\_7000  &  & 1764277         & 1742121.70 &  & 1802880          & 1798430.90         &           & \textbf{1816714}    & \textbf{1816714.00} & 0.00  & 23.069  \\
bmcp\_4200\_4400\_0.3\_10000 &  & 1954069         & 1932251.00 &  & 2022834          & 2016260.10         &           & \textbf{2023093}    & \textbf{2023093.00} & 0.00  & 21.845  \\
bmcp\_4200\_4400\_0.5\_7000  &  & 1853677         & 1820444.40 &  & 1894307          & 1883721.00         &           & \textbf{1903515}    & \textbf{1903515.00} & 0.00  & 17.612  \\
bmcp\_4400\_4200\_0.3\_10000 &  & 1833465         & 1816879.10 &  & 1911617          & 1905971.70         &           & \textbf{1920418}    & \textbf{1920418.00} & 0.00  & 25.126  \\
bmcp\_4400\_4200\_0.5\_7000  &  & 1746064         & 1730783.90 &  & 1807860          & 1799645.50         &           & \textbf{1811179}    & \textbf{1811179.00} & 0.00  & 44.223  \\
bmcp\_4400\_4400\_0.3\_10000 &  & 1945218         & 1922134.20 &  & 2023432          & 2019636.30         &           & \textbf{2028288}    & \textbf{2028288.00} & 0.00  & 4.064   \\
bmcp\_4400\_4400\_0.5\_7000  &  & 1844031         & 1821467.80 &  & 1888693          & 1882463.10         &           & \textbf{1905810}    & \textbf{1905810.00} & 0.00  & 68.641  \\
bmcp\_4400\_4600\_0.3\_10000 &  & 2003959         & 1993946.20 &  & 2097123          & 2088349.10         &           & \textbf{2100925}    & \textbf{2100925.00} & 0.00  & 6.291   \\
bmcp\_4400\_4600\_0.5\_7000  &  & 1937066         & 1906956.10 &  & 1981337          & 1973941.30         &           & \textbf{1991870}    & \textbf{1991870.00} & 0.00  & 8.372   \\
bmcp\_4600\_4400\_0.3\_10000 &  & 1930498         & 1913501.00 &  & \textit{2011730} & 1998707.00         &           & \textit{2011730}    & \textbf{2011730.00} & 0.00  & 11.351  \\
bmcp\_4600\_4400\_0.5\_7000  &  & 1845046         & 1817697.20 &  & 1897119          & 1889599.70         &           & \textbf{1901868}    & \textbf{1901868.00} & 0.00  & 97.821  \\
bmcp\_4600\_4600\_0.3\_10000 &  & 2027132         & 2005096.70 &  & 2103476          & 2093832.30         &           & \textbf{2106970}    & \textbf{2106970.00} & 0.00  & 7.914   \\
bmcp\_4600\_4600\_0.5\_7000  &  & 1921261         & 1900376.30 &  & 1976832          & 1970554.10         &           & \textbf{1984295}    & \textbf{1984295.00} & 0.00  & 41.538  \\
bmcp\_4600\_4800\_0.3\_10000 &  & 2120120         & 2091722.50 &  & 2200580          & 2193619.00         &           & \textbf{2203833}    & \textbf{2203833.00} & 0.00  & 18.406  \\
bmcp\_4600\_4800\_0.5\_7000  &  & 1989454         & 1967943.30 &  & 2064098          & 2053550.30         &           & \textbf{2074036}    & \textbf{2074036.00} & 0.00  & 22.452  \\
bmcp\_4800\_4600\_0.3\_10000 &  & 2019033         & 1991673.50 &  & 2093497          & 2081197.60         &           & \textbf{2101148}    & \textbf{2101148.00} & 0.00  & 10.699  \\
bmcp\_4800\_4600\_0.5\_7000  &  & 1922466         & 1901157.60 &  & 1977557          & 1969484.10         &           & \textbf{1992370}    & \textbf{1992370.00} & 0.00  & 109.582 \\
bmcp\_4800\_4800\_0.3\_10000 &  & 2100773         & 2058921.60 &  & 2180165          & 2171120.60         &           & \textbf{2185367}    & \textbf{2185367.00} & 0.00  & 7.115   \\
bmcp\_4800\_4800\_0.5\_7000  &  & 2009129         & 1973993.60 &  & 2058797          & 2053170.90         &           & \textbf{2075133}    & \textbf{2075133.00} & 0.00  & 346.026 \\
bmcp\_4800\_5000\_0.3\_10000 &  & 2184445         & 2157793.00 &  & 2275455          & 2270224.70         &           & \textbf{2280317}    & \textbf{2280317.00} & 0.00  & 3.414   \\
bmcp\_4800\_5000\_0.5\_7000  &  & 2087596         & 2050741.00 &  & 2133843          & 2129594.00         &           & \textbf{2151715}    & \textbf{2151715.00} & 0.00  & 203.314 \\
bmcp\_5000\_4800\_0.3\_10000 &  & 2069979         & 2051607.20 &  & 2181584          & 2167254.80         &           & \textbf{2184508}    & \textbf{2184508.00} & 0.00  & 11.619  \\
bmcp\_5000\_4800\_0.5\_7000  &  & 2013921         & 1977310.70 &  & 2061909          & 2053025.70         &           & \textbf{2070324}    & \textbf{2070305.90} & 54.30 & 468.996 \\
bmcp\_5000\_5000\_0.3\_10000 &  & 2144223         & 2126462.90 &  & 2254007          & 2247746.10         &           & \textbf{2261620}    & \textbf{2261620.00} & 0.00  & 107.113 \\
bmcp\_5000\_5000\_0.5\_7000  &  & 2067188         & 2046886.50 &  & 2145927          & 2135823.30         &           & \textbf{2151921}    & \textbf{2151921.00} & 0.00  & 32.261  \\
bmcp\_5000\_5200\_0.3\_10000 &  & 2231359         & 2220887.20 &  & 2352676          & 2340288.00         &           & \textbf{2354408}    & \textbf{2354408.00} & 0.00  & 14.278  \\
bmcp\_5000\_5200\_0.5\_7000  &  & 2129556         & 2115338.30 &  & 2224001          & 2207572.40         &           & \textbf{2227362}    & \textbf{2227362.00} & 0.00  & 341.662 \\ \hline
Average                                                            &  & 1967744.97      & 1943665.33 &  & 2037176.70       & 2028758.57         &           & \textbf{2044036.53} & \textbf{2044035.93} & 1.81  & 70.037 \\ \bottomrule
\end{tabular}}
\end{table*}

==> table-SUKP.tex <==
\begin{sidewaystable*}[thp]
\caption{Comparison of E2LS with the baseline algorithms on all the three sets of SUKP instances. Unique best results appear in bold. Equal best results appear in italic.\vspace{-0.3em}}
\label{table-SUKP}
\centering
\scalebox{0.45}{\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrr} \toprule
Instance\textbackslash{}Algorithm &  & \multicolumn{4}{r}{I2PLS}                             &  & \multicolumn{4}{r}{KBTS}                                 &  & \multicolumn{4}{r}{MSBTS}                             &  & \multicolumn{4}{r}{ATS-DLA}                           &  & \multicolumn{4}{r}{E2LS}                                \\ \cline{3-6} \cline{8-11} \cline{13-16} \cline{18-21} \cline{23-26} 
                                  &  & Best           & Average           & S.D.   & Time    &  & Best              & Average           & S.D.   & Time    &  & Best           & Average           & S.D.   & Time    &  & Best           & Average           & S.D.   & Time    &  & Best              & Average           & S.D.  & Time    \\ \hline
\multicolumn{26}{l}{\textit{Set I}}                                                                                                                                                                                                                                                                                                           \\ \hline
sukp\_100\_85\_0.10\_0.75     &  & \textit{13283} & \textit{13283.00} & 0.00   & 0.883   &  & \textit{13283}    & \textit{13283.00} & 0.00   & 3.219   &  & \textit{13283} & \textit{13283.00} & 0.00   & 497.286 &  & 13016          & 12917.50          & 101.70 & 5.477   &  & \textit{13283}    & 13276.60          & 12.80 & 66.663  \\
sukp\_100\_85\_0.15\_0.85     &  & \textit{12479} & 12361.10          & 128.09 & 42.547  &  & \textit{12479}    & \textbf{12479.00} & 0.00   & 22.052  &  & \textit{12479} & 12445.40          & 69.21  & 498.053 &  & 11902          & 11400.20          & 369.75 & 0.013   &  & \textit{12479}    & 12456.70          & 55.14 & 134.929 \\
sukp\_200\_185\_0.10\_0.75    &  & \textit{13521} & \textit{13521.00} & 0.00   & 50.447  &  & \textit{13521}    & \textit{13521.00} & 0.00   & 0.884   &  & \textit{13521} & \textit{13521.00} & 0.00   & 406.291 &  & \textit{13521} & \textit{13521.00} & 0.00   & 51.034  &  & \textit{13521}    & \textit{13521.00} & 0.00  & 17.815  \\
sukp\_200\_185\_0.15\_0.85    &  & \textit{14215} & 14044.40          & 62.18  & 172.901 &  & \textit{14215}    & \textit{14215.00} & 0.00   & 143.365 &  & \textit{14215} & 14038.40          & 132.04 & 458.665 &  & \textit{14215} & 13913.10          & 233.49 & 3.690   &  & \textit{14215}    & \textit{14215.00} & 0.00  & 7.355   \\
sukp\_300\_285\_0.10\_0.75    &  & \textit{11563} & \textit{11563.00} & 0.00   & 97.453  &  & \textit{11563}    & \textit{11563.00} & 0.00   & 21.066  &  & \textit{11563} & \textit{11563.00} & 0.00   & 18.615  &  & \textit{11563} & \textit{11563.00} & 0.00   & 6.256   &  & \textit{11563}    & \textit{11563.00} & 0.00  & 6.576   \\
sukp\_300\_285\_0.15\_0.85    &  & 12402          & 12343.40          & 44.66  & 159.279 &  & \textit{12607}    & 12536.02          & 87.51  & 247.327 &  & 12500          & 12419.00          & 27.13  & 168.993 &  & 12500          & 12500.00          & 0.00   & 175.921 &  & \textit{12607}    & \textbf{12564.20} & 52.42 & 247.200 \\
sukp\_400\_385\_0.10\_0.75    &  & \textit{11484} & \textit{11484.00} & 0.00   & 22.326  &  & \textit{11484}    & \textit{11484.00} & 0.00   & 8.047   &  & \textit{11484} & \textit{11484.00} & 0.00   & 1.022   &  & \textit{11484} & \textit{11484.00} & 0.00   & 0.903   &  & \textit{11484}    & \textit{11484.00} & 0.00  & 5.115   \\
sukp\_400\_385\_0.15\_0.85    &  & \textit{11209} & 11169.20          & 79.60  & 73.640  &  & \textit{11209}    & \textit{11209.00} & 0.00   & 48.967  &  & \textit{11209} & \textit{11209.00} & 0.00   & 35.043  &  & \textit{11209} & \textit{11209.00} & 0.00   & 2.347   &  & \textit{11209}    & 11165.00          & 47.24 & 228.405 \\
sukp\_500\_485\_0.10\_0.75    &  & 11729          & 11729.00          & 0.00   & 100.289 &  & \textit{11771}    & 11762.60          & 16.80  & 188.023 &  & \textit{11771} & \textit{11771.00} & 0.00   & 15.251  &  & \textit{11771} & \textit{11771.00} & 0.00   & 16.260  &  & \textit{11771}    & \textit{11771.00} & 0.00  & 5.891   \\
sukp\_500\_485\_0.15\_0.85    &  & 10217          & 10164.80          & 50.08  & 223.788 &  & \textit{10238}    & 10209.50          & 19.84  & 127.369 &  & \textit{10238} & 10214.50          & 11.99  & 200.523 &  & \textit{10238} & \textit{10238.00} & 0.00   & 22.116  &  & \textit{10238}    & \textit{10238.00} & 0.00  & 67.571  \\
sukp\_100\_100\_0.10\_0.75    &  & \textit{14044} & \textit{14044.00} & 0.00   & 32.919  &  & \textit{14044}    & \textit{14044.00} & 0.00   & 4.254   &  & \textit{14044} & \textit{14044.00} & 0.00   & 495.768 &  & \textit{14044} & \textit{14044.00} & 0.00   & 0.280   &  & \textit{14044}    & \textit{14044.00} & 0.00  & 0.604   \\
sukp\_100\_100\_0.15\_0.85    &  & \textit{13508} & 13485.80          & 39.59  & 36.227  &  & \textit{13508}    & \textit{13508.00} & 0.00   & 14.357  &  & \textit{13508} & \textit{13508.00} & 0.00   & 493.352 &  & 13370          & 12636.30          & 518.83 & 0.012   &  & \textit{13508}    & \textit{13508.00} & 0.00  & 10.898  \\
sukp\_200\_200\_0.10\_0.75    &  & \textit{12522} & \textit{12522.00} & 0.00   & 20.781  &  & \textit{12522}    & \textit{12522.00} & 0.00   & 30.710  &  & \textit{12522} & \textit{12522.00} & 0.00   & 454.370 &  & \textit{12522} & \textit{12522.00} & 0.00   & 9.358   &  & \textit{12522}    & \textit{12522.00} & 0.00  & 11.155  \\
sukp\_200\_200\_0.15\_0.85    &  & \textit{12317} & 12275.60          & 53.03  & 202.722 &  & \textit{12317}    & \textit{12317.00} & 0.00   & 38.887  &  & \textit{12317} & \textit{12317.00} & 0.00   & 389.541 &  & \textit{12317} & \textit{12317.00} & 0.00   & 4.462   &  & \textit{12317}    & \textit{12317.00} & 0.00  & 11.395  \\
sukp\_300\_300\_0.10\_0.75    &  & \textit{12817} & \textit{12817.00} & 0.00   & 55.855  &  & \textit{12817}    & \textit{12817.00} & 0.00   & 40.194  &  & \textit{12817} & 12813.70          & 9.90   & 117.170 &  & \textit{12817} & \textit{12817.00} & 0.00   & 2.199   &  & \textit{12817}    & \textit{12817.00} & 0.00  & 7.965   \\
sukp\_300\_300\_0.15\_0.85    &  & \textit{11585} & 11523.50          & 75.57  & 133.364 &  & \textit{11585}    & \textit{11585.00} & 0.00   & 136.511 &  & \textit{11585} & 11576.50          & 25.50  & 135.658 &  & \textit{11585} & \textit{11585.00} & 0.00   & 1.513   &  & \textit{11585}    & \textit{11585.00} & 0.00  & 27.443  \\
sukp\_400\_400\_0.10\_0.75    &  & \textit{11665} & \textit{11665.00} & 0.00   & 16.181  &  & \textit{11665}    & \textit{11665.00} & 0.00   & 118.757 &  & \textit{11665} & 11651.80          & 10.78  & 86.003  &  & \textit{11665} & \textit{11665.00} & 0.00   & 8.623   &  & \textit{11665}    & \textit{11665.00} & 0.00  & 2.198   \\
sukp\_400\_400\_0.15\_0.85    &  & \textit{11325} & \textit{11325.00} & 0.00   & 37.422  &  & \textit{11325}    & \textit{11325.00} & 0.00   & 5.981   &  & \textit{11325} & 11260.40          & 193.80 & 102.850 &  & \textit{11325} & \textit{11325.00} & 0.00   & 1.010   &  & \textit{11325}    & \textit{11325.00} & 0.00  & 8.239   \\
sukp\_500\_500\_0.10\_0.75    &  & \textit{11249} & \textit{11249.00} & 0.00   & 80.338  &  & \textit{11249}    & \textit{11249.00} & 0.00   & 94.334  &  & \textit{11249} & \textit{11249.00} & 0.00   & 19.433  &  & \textit{11249} & \textit{11249.00} & 0.00   & 3.085   &  & \textit{11249}    & \textit{11249.00} & 0.00  & 6.632   \\
sukp\_500\_500\_0.15\_0.85    &  & \textit{10381} & 10313.00          & 83.35  & 181.218 &  & \textit{10381}    & 10364.30          & 50.10  & 155.402 &  & \textit{10381} & 10359.80          & 63.60  & 192.505 &  & \textit{10381} & \textit{10381.00} & 0.00   & 4.152   &  & \textit{10381}    & \textit{10381.00} & 0.00  & 39.511  \\
sukp\_85\_100\_0.10\_0.75     &  & \textit{12045} & \textit{12045.00} & 0.00   & 2.200   &  & \textit{12045}    & \textit{12045.00} & 0.00   & 1.225   &  & \textit{12045} & \textit{12045.00} & 0.00   & 497.513 &  & \textit{12045} & \textit{12045.00} & 0.00   & 0.164   &  & \textit{12045}    & \textit{12045.00} & 0.00  & 0.328   \\
sukp\_85\_100\_0.15\_0.85     &  & \textit{12369} & 12327.00          & 34.29  & 4.130   &  & \textit{12369}    & \textit{12369.00} & 0.00   & 0.490   &  & \textit{12369} & \textit{12369.00} & 0.00   & 498.611 &  & 12224          & 11811.00          & 266.98 & 0.028   &  & \textit{12369}    & \textit{12369.00} & 0.00  & 132.154 \\
sukp\_185\_200\_0.10\_0.75    &  & \textit{13696} & 13695.90          & 0.30   & 130.039 &  & \textit{13696}    & \textit{13696.00} & 0.00   & 8.606   &  & \textit{13696} & \textit{13696.00} & 0.00   & 439.130 &  & \textit{13696} & \textit{13696.00} & 0.00   & 0.973   &  & \textit{13696}    & 13695.90          & 0.30  & 76.578  \\
sukp\_185\_200\_0.15\_0.85    &  & \textit{11298} & \textit{11298.00} & 0.00   & 123.179 &  & \textit{11298}    & \textit{11298.00} & 0.00   & 0.716   &  & \textit{11298} & \textit{11298.00} & 0.00   & 424.992 &  & \textit{11298} & \textit{11298.00} & 0.00   & 2.962   &  & \textit{11298}    & \textit{11298.00} & 0.00  & 0.684   \\
sukp\_285\_300\_0.10\_0.75    &  & \textit{11568} & \textit{11568.00} & 0.00   & 4.595   &  & \textit{11568}    & \textit{11568.00} & 0.00   & 40.810  &  & \textit{11568} & \textit{11568.00} & 0.00   & 11.030  &  & \textit{11568} & \textit{11568.00} & 0.00   & 2.237   &  & \textit{11568}    & \textit{11568.00} & 0.00  & 0.945   \\
sukp\_285\_300\_0.15\_0.85    &  & \textit{11802} & 11798.10          & 11.70  & 204.408 &  & \textit{11802}    & \textit{11802.00} & 0.00   & 134.096 &  & \textit{11802} & \textit{11802.00} & 0.00   & 151.069 &  & \textit{11802} & \textit{11802.00} & 0.00   & 4.856   &  & \textit{11802}    & \textit{11802.00} & 0.00  & 54.879  \\
sukp\_385\_400\_0.10\_0.75    &  & \textit{10600} & 10533.80          & 54.05  & 139.626 &  & \textit{10600}    & \textit{10600.00} & 0.00   & 43.289  &  & \textit{10600} & \textit{10599.00} & 3.00   & 130.469 &  & \textit{10600} & \textit{10600.00} & 0.00   & 13.548  &  & \textit{10600}    & \textit{10600.00} & 0.00  & 52.287  \\
sukp\_385\_400\_0.15\_0.85    &  & \textit{10506} & \textit{10506.00} & 0.00   & 117.813 &  & \textit{10506}    & \textit{10506.00} & 0.00   & 1.503   &  & \textit{10506} & \textit{10506.00} & 0.00   & 118.308 &  & \textit{10506} & \textit{10506.00} & 0.00   & 2.095   &  & \textit{10506}    & \textit{10506.00} & 0.00  & 11.861  \\
sukp\_485\_500\_0.10\_0.75    &  & \textit{11321} & 11313.80          & 14.40  & 113.786 &  & \textit{11321}    & \textit{11321.00} & 0.00   & 100.472 &  & \textit{11321} & \textit{11321.00} & 0.00   & 64.100  &  & \textit{11321} & \textit{11321.00} & 0.00   & 3.523   &  & \textit{11321}    & \textit{11321.00} & 0.00  & 16.619  \\
sukp\_485\_500\_0.15\_0.85    &  & \textit{10220} & 10174.60          & 46.02  & 141.829 &  & \textit{10220}    & \textit{10220.00} & 0.00   & 10.494  &  & \textit{10220} & 10218.80          & 3.60   & 100.407 &  & \textit{10220} & \textit{10220.00} & 0.00   & 1.694   &  & \textit{10220}    & \textit{10220.00} & 0.00  & 5.297   \\ \hline
Average                           &  & 11964.67       & 11938.10          & 25.90  & 90.740  &  & \textit{11973.60} & 11969.45          & 5.81   & 59.714  &  & 11970.03       & 11955.78          & 18.35  & 240.734 &  & 11932.47       & 11864.17          & 49.69  & 11.693  &  & \textit{11973.60} & \textbf{11969.75} & 5.60  & 42.173  \\ \hline
\multicolumn{26}{l}{\textit{Set II}}                                                                                                                                                                                                                                                                                                          \\ \hline
sukp\_600\_585\_0.10\_0.75    &  & 9750           & 9731.50           & 12.64  & 315.869 &  & \textit{9914}     & \textit{9914.00}  & 0.00   & 183.513 &  & \textit{9914}  & \textit{9914.00}  & 0.00   & 152.437 &  & 9790           & 9746.70           & 14.46  & 269.974 &  & \textit{9914}     & \textit{9914.00}  & 0.00  & 16.191  \\
sukp\_600\_585\_0.15\_0.85    &  & \textit{9357}  & 9320.00           & 14.57  & 189.829 &  & \textit{9357}     & \textit{9357.00}  & 0.00   & 370.468 &  & \textit{9357}  & \textit{9357.00}  & 0.00   & 49.735  &  & \textit{9357}  & \textit{9357.00}  & 0.00   & 4.552   &  & \textit{9357}     & \textit{9357.00}  & 0.00  & 27.229  \\
sukp\_700\_685\_0.10\_0.75    &  & \textit{9881}  & 9814.80           & 43.61  & 328.507 &  & \textit{9881}     & 9853.00           & 18.33  & 244.831 &  & \textit{9881}  & \textit{9881.00}  & 0.00   & 22.714  &  & \textit{9881}  & \textit{9881.00}  & 0.00   & 1.810   &  & \textit{9881}     & \textit{9881.00}  & 0.00  & 16.557  \\
sukp\_700\_685\_0.15\_0.85    &  & 9135           & 9135.00           & 0.00   & 249.852 &  & \textit{9163}     & 9140.60           & 11.20  & 197.666 &  & \textit{9163}  & \textit{9163.00}  & 0.00   & 82.473  &  & \textit{9163}  & \textit{9163.00}  & 0.00   & 4.877   &  & \textit{9163}     & \textit{9163.00}  & 0.00  & 60.807  \\
sukp\_800\_785\_0.10\_0.75    &  & 9822           & 9745.80           & 61.06  & 444.098 &  & 9837              & 9816.20           & 13.91  & 363.597 &  & \textit{9937}  & \textit{9937.00}  & 0.00   & 162.069 &  & \textit{9937}  & \textit{9937.00}  & 0.00   & 6.238   &  & \textit{9937}     & \textit{9937.00}  & 0.00  & 18.053  \\
sukp\_800\_785\_0.15\_0.85    &  & 8803           & 8772.40           & 22.15  & 297.988 &  & 8969              & 8928.70           & 13.48  & 503.634 &  & \textit{9024}  & 9002.00           & 26.94  & 326.235 &  & \textit{9024}  & \textit{9024.00}  & 0.00   & 187.296 &  & \textit{9024}     & \textit{9024.00}  & 0.00  & 7.556   \\
sukp\_900\_885\_0.10\_0.75    &  & 9611           & 9517.10           & 49.81  & 283.090 &  & \textit{9725}     & 9622.40           & 34.20  & 197.352 &  & \textit{9725}  & \textit{9725.00}  & 0.00   & 148.120 &  & \textit{9725}  & \textit{9725.00}  & 0.00   & 1.388   &  & \textit{9725}     & \textit{9725.00}  & 0.00  & 2.751   \\
sukp\_900\_885\_0.15\_0.85    &  & 8481           & 8448.60           & 37.87  & 542.880 &  & 8588              & 8532.10           & 46.82  & 491.230 &  & 8588           & 8588.00           & 0.00   & 626.844 &  & \textit{8620}  & \textit{8620.00}  & 0.00   & 90.409  &  & \textit{8620}     & \textit{8620.00}  & 0.00  & 38.149  \\
sukp\_1000\_985\_0.10\_0.75   &  & 9447           & 9225.40           & 90.95  & 128.051 &  & 9668              & 9487.40           & 71.13  & 345.018 &  & \textit{9689}  & 9637.10           & 30.07  & 526.307 &  & \textit{9689}  & \textit{9689.00}  & 0.00   & 38.096  &  & \textit{9689}     & \textit{9689.00}  & 0.00  & 57.874  \\
sukp\_1000\_985\_0.15\_0.85   &  & 8448           & 8248.50           & 130.60 & 264.180 &  & 8448              & 8448.00           & 0.00   & 3.013   &  & \textit{8455}  & 8453.40           & 0.80   & 433.914 &  & \textit{8455}  & \textit{8455.00}  & 0.00   & 254.163 &  & \textit{8455}     & \textit{8455.00}  & 0.00  & 29.703  \\
sukp\_600\_600\_0.10\_0.75    &  & \textit{10524} & 10520.40          & 2.94   & 214.709 &  & \textit{10524}    & 10522.80          & 2.40   & 286.020 &  & \textit{10524} & \textit{10524.00} & 0.00   & 11.461  &  & \textit{10524} & \textit{10524.00} & 0.00   & 1.737   &  & \textit{10524}    & \textit{10524.00} & 0.00  & 3.977   \\
sukp\_600\_600\_0.15\_0.85    &  & \textit{9062}  & 9042.90           & 25.72  & 553.782 &  & \textit{9062}     & \textit{9062.00}  & 0.00   & 305.532 &  & \textit{9062}  & \textit{9062.00}  & 0.00   & 193.985 &  & \textit{9062}  & \textit{9062.00}  & 0.00   & 59.618  &  & \textit{9062}     & \textit{9062.00}  & 0.00  & 77.862  \\
sukp\_700\_700\_0.10\_0.75    &  & \textit{9786}  & 9750.00           & 23.75  & 491.156 &  & \textit{9786}     & \textit{9786.00}  & 0.00   & 59.776  &  & \textit{9786}  & \textit{9786.00}  & 0.00   & 44.334  &  & \textit{9786}  & \textit{9786.00}  & 0.00   & 4.276   &  & \textit{9786}     & 9785.60           & 0.80  & 327.675 \\
sukp\_700\_700\_0.15\_0.85    &  & \textit{9229}  & 9161.50           & 22.50  & 315.183 &  & \textit{9229}     & 9187.40           & 20.80  & 223.412 &  & \textit{9229}  & \textit{9229.00}  & 0.00   & 90.435  &  & \textit{9229}  & \textit{9229.00}  & 0.00   & 5.179   &  & \textit{9229}     & \textit{9229.00}  & 0.00  & 49.776  \\
sukp\_800\_800\_0.10\_0.75    &  & 9718           & 9687.00           & 65.75  & 197.777 &  & \textit{9932}     & \textit{9932.00}  & 0.00   & 196.482 &  & \textit{9932}  & \textit{9932.00}  & 0.00   & 16.074  &  & \textit{9932}  & \textit{9932.00}  & 0.00   & 2.180   &  & \textit{9932}     & \textit{9932.00}  & 0.00  & 2.147   \\
sukp\_800\_800\_0.15\_0.85    &  & 8961           & 8917.30           & 20.63  & 150.903 &  & \textit{9101}     & 8936.20           & 58.23  & 176.002 &  & \textit{9101}  & \textit{9101.00}  & 0.00   & 125.276 &  & \textit{9101}  & \textit{9101.00}  & 0.00   & 0.093   &  & \textit{9101}     & \textit{9101.00}  & 0.00  & 5.154   \\
sukp\_900\_900\_0.10\_0.75    &  & 9660           & 9657.60           & 7.20   & 426.406 &  & \textit{9745}     & \textit{9745.00}  & 0.00   & 421.663 &  & \textit{9745}  & \textit{9745.00}  & 0.00   & 26.282  &  & \textit{9745}  & \textit{9745.00}  & 0.00   & 3.325   &  & \textit{9745}     & \textit{9745.00}  & 0.00  & 8.761   \\
sukp\_900\_900\_0.15\_0.85    &  & 8916           & 8916.00           & 0.00   & 115.926 &  & 8916              & 8916.00           & 0.00   & 9.104   &  & \textit{8990}  & \textit{8990.00}  & 0.00   & 160.114 &  & \textit{8990}  & \textit{8990.00}  & 0.00   & 2.939   &  & \textit{8990}     & \textit{8990.00}  & 0.00  & 14.542  \\
sukp\_1000\_1000\_0.10\_0.75  &  & 9414           & 9318.20           & 117.43 & 441.503 &  & 9544              & 9453.00           & 59.57  & 254.001 &  & \textit{9551}  & \textit{9551.00}  & 0.00   & 118.014 &  & \textit{9551}  & \textit{9551.00}  & 0.00   & 2.083   &  & \textit{9551}     & \textit{9551.00}  & 0.00  & 2.495   \\
sukp\_1000\_1000\_0.15\_0.85  &  & 8184           & 8181.20           & 8.40   & 374.563 &  & \textit{8538}     & 8396.70           & 47.10  & 209.621 &  & \textit{8538}  & 8495.10           & 26.17  & 506.568 &  & \textit{8538}  & \textit{8538.00}  & 0.00   & 39.482  &  & \textit{8538}     & \textit{8538.00}  & 0.00  & 15.148  \\
sukp\_585\_600\_0.10\_0.75    &  & \textit{10393} & 10381.20          & 23.60  & 259.802 &  & \textit{10393}    & \textit{10393.00} & 0.00   & 41.564  &  & \textit{10393} & \textit{10393.00} & 0.00   & 54.925  &  & \textit{10393} & \textit{10393.00} & 0.00   & 0.588   &  & \textit{10393}    & \textit{10393.00} & 0.00  & 6.340   \\
sukp\_585\_600\_0.15\_0.85    &  & \textit{9256}  & \textit{9256.00}  & 0.00   & 228.666 &  & \textit{9256}     & \textit{9256.00}  & 0.00   & 91.279  &  & \textit{9256}  & \textit{9256.00}  & 0.00   & 78.201  &  & \textit{9256}  & \textit{9256.00}  & 0.00   & 4.647   &  & \textit{9256}     & \textit{9256.00}  & 0.00  & 9.692   \\
sukp\_685\_700\_0.10\_0.75    &  & \textit{10121} & 9985.70           & 88.64  & 184.425 &  & \textit{10121}    & \textit{10121.00} & 0.00   & 183.002 &  & \textit{10121} & \textit{10121.00} & 0.00   & 6.954   &  & \textit{10121} & \textit{10121.00} & 0.00   & 0.471   &  & \textit{10121}    & \textit{10121.00} & 0.00  & 0.983   \\
sukp\_685\_700\_0.15\_0.85    &  & \textit{9176}  & 9155.70           & 35.50  & 368.305 &  & \textit{9176}     & \textit{9176.00}  & 0.00   & 65.660  &  & \textit{9176}  & \textit{9176.00}  & 0.00   & 144.591 &  & \textit{9176}  & \textit{9176.00}  & 0.00   & 3.622   &  & \textit{9176}     & 9166.40           & 4.80  & 117.093 \\
sukp\_785\_800\_0.10\_0.75    &  & \textit{9384}  & 9245.60           & 98.15  & 359.349 &  & \textit{9384}     & \textit{9384.00}  & 0.00   & 70.444  &  & \textit{9384}  & \textit{9384.00}  & 0.00   & 173.674 &  & \textit{9384}  & \textit{9384.00}  & 0.00   & 2.476   &  & \textit{9384}     & \textit{9384.00}  & 0.00  & 9.715   \\
sukp\_785\_800\_0.15\_0.85    &  & 8663           & 8556.50           & 70.64  & 540.826 &  & \textit{8746}     & 8652.40           & 43.08  & 554.904 &  & \textit{8746}  & 8687.90           & 38.04  & 328.837 &  & \textit{8746}  & \textit{8746.00}  & 0.00   & 53.519  &  & \textit{8746}     & \textit{8746.00}  & 0.00  & 131.179 \\
sukp\_885\_900\_0.10\_0.75    &  & 9184           & 9124.10           & 49.57  & 454.128 &  & \textit{9318}     & 9257.80           & 39.41  & 161.452 &  & \textit{9318}  & \textit{9318.00}  & 0.00   & 69.982  &  & \textit{9318}  & \textit{9318.00}  & 0.00   & 10.103  &  & \textit{9318}     & \textit{9318.00}  & 0.00  & 25.416  \\
sukp\_885\_900\_0.15\_0.85    &  & \textit{8425}  & 8276.60           & 51.68  & 401.835 &  & \textit{8425}     & 8337.80           & 61.02  & 417.072 &  & \textit{8425}  & 8413.80           & 7.33   & 281.830 &  & \textit{8425}  & \textit{8425.00}  & 0.00   & 105.995 &  & \textit{8425}     & \textit{8425.00}  & 0.00  & 77.413  \\
sukp\_985\_1000\_0.10\_0.75   &  & 8990           & 8960.80           & 87.60  & 533.984 &  & 9186              & 9115.80           & 66.85  & 351.768 &  & \textit{9234}  & 9198.40           & 18.07  & 502.731 &  & \textit{9234}  & \textit{9234.00}  & 0.00   & 10.962  &  & \textit{9234}     & \textit{9234.00}  & 0.00  & 28.558  \\
sukp\_985\_1000\_0.15\_0.85   &  & 8453           & 8273.90           & 115.97 & 338.731 &  & 8528              & 8492.70           & 32.11  & 325.071 &  & \textit{8612}  & 8560.00           & 26.00  & 155.412 &  & \textit{8612}  & \textit{8612.00}  & 0.00   & 26.441  &  & \textit{8612}     & \textit{8612.00}  & 0.00  & 18.267  \\ \hline
Average                           &  & 9274.47        & 9210.91           & 45.96  & 333.210 &  & 9348.67           & 9307.43           & 21.32  & 243.472 &  & 9361.87        & 9352.69           & 5.78   & 187.351 &  & 9358.80        & 9357.36           & 0.48   & 39.951  &  & \textbf{9362.93}  & \textbf{9362.60}  & 0.19  & 40.235  \\ \hline
\multicolumn{26}{l}{\textit{Set III}}                                                                                                                                                                                                                                                                                                         \\ \hline
sukp\_850\_1000\_0.10\_0.75   &  & 9944           & 9851.90           & 96.12  & 454.059 &  & 9983              & 9942.20           & 21.77  & 183.600 &  & \textit{10028} & \textit{10028.00} & 0.00   & 189.841 &  & \textit{10028} & \textit{10028.00} & 0.00   & 16.553  &  & \textit{10028}    & \textit{10028.00} & 0.00  & 85.080  \\
sukp\_850\_1000\_0.15\_0.85   &  & 8851           & 8838.30           & 22.52  & 355.332 &  & \textit{8957}     & 8919.10           & 17.82  & 173.008 &  & \textit{8957}  & \textit{8957.00}  & 0.00   & 356.205 &  & \textit{8957}  & \textit{8957.00}  & 0.00   & 17.191  &  & \textit{8957}     & \textit{8957.00}  & 0.00  & 39.932  \\
sukp\_1000\_850\_0.10\_0.75   &  & 10464          & 10434.30          & 46.83  & 344.512 &  & \textit{10623}    & 10610.40          & 10.29  & 309.152 &  & \textit{10623} & \textit{10623.00} & 0.00   & 385.623 &  & 10511          & 10403.80          & 39.10  & 343.725 &  & \textit{10623}    & \textit{10623.00} & 0.00  & 51.127  \\
sukp\_1000\_850\_0.15\_0.85   &  & 9532           & 9394.70           & 95.33  & 578.656 &  & 9503              & 9487.50           & 9.33   & 426.328 &  & \textit{9565}  & 9546.00           & 25.01  & 255.350 &  & 9451           & 9436.60           & 11.76  & 325.252 &  & \textit{9565}     & \textbf{9565.00}  & 0.00  & 69.196  \\
sukp\_1000\_1000\_0.10\_0.75  &  & 10723          & 10515.40          & 88.34  & 400.805 &  & 10607             & 10585.30          & 47.87  & 381.060 &  & \textit{10771} & \textit{10771.00} & 0.00   & 183.362 &  & \textit{10771} & \textit{10771.00} & 0.00   & 2.323   &  & \textit{10771}    & \textit{10771.00} & 0.00  & 3.319   \\
sukp\_1000\_1000\_0.15\_0.85  &  & 9342           & 9235.00           & 142.12 & 212.259 &  & 9342              & 9316.70           & 25.38  & 193.854 &  & \textit{9368}  & 9344.80           & 7.74   & 269.884 &  & \textit{9368}  & \textit{9368.00}  & 0.00   & 82.009  &  & \textit{9368}     & \textit{9368.00}  & 0.00  & 253.839 \\
sukp\_2850\_3000\_0.10\_0.75  &  & 8206           & 8206.00           & 0.00   & 76.246  &  & 9159              & 9153.30           & 4.41   & 80.165  &  & 8709           & 8507.80           & 246.42 & 6.076   &  & \textit{9260}  & \textbf{9260.00}  & 0.00   & 275.973 &  & \textit{9260}     & 9256.50           & 7.99  & 484.974 \\
sukp\_2850\_3000\_0.15\_0.85  &  & 7132           & 7132.00           & 0.00   & 62.363  &  & 8061              & 8050.50           & 6.09   & 105.651 &  & 7639           & 7334.80           & 248.38 & 2.537   &  & \textit{8066}  & \textbf{8062.50}  & 2.29   & 357.251 &  & \textit{8066}     & 8057.70           & 6.07  & 522.812 \\
sukp\_3000\_2850\_0.10\_0.75  &  & 8192           & 8191.90           & 0.30   & 110.108 &  & 8991              & 8989.20           & 5.40   & 51.555  &  & 8665           & 8239.30           & 141.90 & 16.185  &  & 8972           & 8944.50           & 14.85  & 236.314 &  & \textbf{9097}     & \textbf{9096.20}  & 0.98  & 234.154 \\
sukp\_3000\_2850\_0.15\_0.85  &  & 7132           & 7131.80           & 0.40   & 373.425 &  & 8072              & 8072.00           & 0.00   & 59.926  &  & 7632           & 7532.00           & 200.00 & 33.481  &  & 8148           & 8092.80           & 45.07  & 389.701 &  & \textbf{8282}     & \textbf{8282.00}  & 0.00  & 49.803  \\
sukp\_3000\_3000\_0.10\_0.75  &  & 8206           & 8204.70           & 1.62   & 108.057 &  & 9104              & 9097.10           & 10.54  & 144.336 &  & 8703           & 8355.10           & 227.75 & 4.086   &  & \textit{9175}  & \textit{9175.00}  & 0.00   & 45.149  &  & \textit{9175}     & \textit{9175.00}  & 0.00  & 96.435  \\
sukp\_3000\_3000\_0.15\_0.85  &  & 7634           & 7632.00           & 4.00   & 135.629 &  & 8026              & 8026.00           & 0.00   & 100.449 &  & 7634           & 7328.60           & 249.36 & 21.276  &  & \textit{8064}  & \textbf{8057.50}  & 9.61   & 321.286 &  & \textit{8064}     & 8037.60           & 16.48 & 351.680 \\
sukp\_4850\_5000\_0.10\_0.75  &  & 9199           & 9199.00           & 0.00   & 541.561 &  & \textit{9480}     & \textit{9480.00}  & 0.00   & 4.408   &  & 8744           & 8692.00           & 156.00 & 43.273  &  & \textit{9480}  & \textit{9480.00}  & 0.00   & 29.943  &  & \textit{9480}     & \textit{9480.00}  & 0.00  & 51.707  \\
sukp\_4850\_5000\_0.15\_0.85  &  & 7676           & 7676.00           & 0.00   & 303.929 &  & 8123              & 8123.00           & 0.00   & 6.354   &  & 7676           & 7676.00           & 0.00   & 3.303   &  & \textit{8226}  & 8171.70           & 45.38  & 407.591 &  & \textit{8226}     & \textbf{8226.00}  & 0.00  & 185.476 \\
sukp\_5000\_4850\_0.10\_0.75  &  & 8731           & 8730.70           & 0.90   & 517.407 &  & 9139              & 9139.00           & 0.00   & 122.712 &  & 8731           & 8578.90           & 232.34 & 16.465  &  & 9139           & 9139.00           & 0.00   & 278.528 &  & \textbf{9207}     & \textbf{9176.60}  & 33.20 & 431.855 \\
sukp\_5000\_4850\_0.15\_0.85  &  & 7653           & 7648.70           & 4.00   & 345.595 &  & \textit{8085}     & \textbf{8085.00}  & 0.00   & 3.161   &  & 7653           & 7549.60           & 206.80 & 67.138  &  & 8082           & 8075.50           & 6.50   & 490.084 &  & \textit{8085}     & 8082.00           & 1.10  & 364.627 \\
sukp\_5000\_5000\_0.10\_0.75  &  & 8226           & 8226.00           & 0.00   & 178.496 &  & \textit{9092}     & 8988.60           & 72.62  & 67.621  &  & 8720           & 8473.00           & 247.00 & 12.723  &  & \textit{9092}  & \textbf{9092.00}  & 0.00   & 163.881 &  & \textit{9092}     & 9084.20           & 12.09 & 358.660 \\
sukp\_5000\_5000\_0.15\_0.85  &  & 7660           & 7660.00           & 0.00   & 264.124 &  & \textit{8090}     & 8028.30           & 185.10 & 243.875 &  & 7660           & 7607.60           & 157.20 & 6.148   &  & \textit{8090}  & 8086.70           & 3.04   & 470.453 &  & \textit{8090}     & \textbf{8088.30}  & 2.45  & 462.180 \\ \hline
Average                           &  & 8583.50        & 8550.47           & 27.91  & 297.920 &  & 9024.28           & 9005.18           & 23.14  & 147.623 &  & 8748.78        & 8619.14           & 130.33 & 104.053 &  & 9048.89        & 9033.42           & 9.87   & 236.289 &  & \textbf{9079.78}  & \textbf{9075.23}  & 4.46  & 227.603 \\ \bottomrule
\end{tabular}}
\end{sidewaystable*}


